Yet Another Pacman 3D Adventures

This game is meant to be extension of the overly-beaten pacman-style game (code-named "Yet Another Pacman 3D Adventures", or YAP3DAD) from the proposed ideas and other projects with advance visual and computer graphics features, including a-game-in-a-game approach. The project is an open-source project published on SourceForge.net for possible future development and extension.

==> references.tex <==
%\addcontentsline{toc}{chapter}{References}

\bibliography{report}
\bibliographystyle{alpha}

% EOF


==> toc.tex <==
\pagenumbering{roman}
\tableofcontents
\clearpage
\pagenumbering{arabic}

\listoffigures
% \listoftables

